High-Dimensional Geometric Streaming for Nearly Low Rank Data

We study streaming algorithms for the $\ell_p$ subspace approximation problem. Given points $a_1, \ldots, a_n$ as an insertion-only stream and a rank parameter $k$, the $\ell_p$ subspace approximation problem is to find a $k$-dimensional subspace $V$ such that $(\sum_{i=1}^n d(a_i, V)^p)^{1/p}$ is minimized, where $d(a, V)$ denotes the Euclidean distance between $a$ and $V$ defined as $\min_{v \in V}\|{a - v}\|_{\infty}$. When $p = \infty$, we need to find a subspace $V$ that minimizes $\max_i d(a_i, V)$. For $\ell_{\infty}$ subspace approximation, we give a deterministic strong coreset construction algorithm and show that it can be used to compute a $\text{poly}(k, \log n)$ approximate solution. We show that the distortion obtained by our coreset is nearly tight for any sublinear space algorithm. For $\ell_p$ subspace approximation, we show that suitably scaling the points and then using our $\ell_{\infty}$ coreset construction, we can compute a $\text{poly}(k, \log n)$ approximation. Our algorithms are easy to implement and run very fast on large datasets. We also use our strong coreset construction to improve the results in a recent work of Woodruff and Yasuda (FOCS 2022) which gives streaming algorithms for high-dimensional geometric problems such as width estimation, convex hull estimation, and volume estimation.

==> adversarial.tex <==
Consider the problem of outputting estimates to the online $\ell_p$ sensitivities. Such an algorithm can be used to identify ``outlier'' rows or rows ``with large leverage" in a data stream.  Algorithm~\ref{alg:one-pass-arbitrary-order} computes these approximations and then samples rows to compute a subspace embedding. We show that a version of our algorithm that just outputs the sensitivity approximations is robust to adversaries.

In our algorithm, we use $O(d \log n)$ wise independent exponential random variables to construct an $\ell_p \rightarrow \ell_{\infty}$ embedding and then use a deterministic $\ell_{\infty}$ coreset construction which we use to compute approximate $\ell_p$ sensitivities. Outputting these estimates directly leaks the information about the exponential random variables which makes the algorithm not robust to adversaries. We argue that by running multiple exponential sketches concurrently and switching to a new sketch to compute approximate sensitivities when the old sketch becomes ``stale'', we can make the algorithm robust to adversaries while outputting $\poly(d, \log n, \log \kappa^{\OL})$ approximations to the online sensitivities. This is inspired by the sketch-switching technique of \cite{ben2022framework}.


==> alternate.tex <==
In Algorithm~\ref{alg:one-pass-arbitrary-order}, we use exponential random variables to embed $\ell_p$ into $\ell_{\infty}$ and then use a coreset of the embedding to compute overestimates for the offline $\ell_p$ sensitivity of a row in the stream. The crucial idea there is that only the ``last'' occurrence of a copy of the row is given a chance to be sampled and as the probability computation is independent of the sampled matrix, the algorithm can be seen as just offline $\ell_p$ sensitivity sampling with estimates being supplied by the exponential embedding. 

An alternate algorithm based on our idea of deleting a previously sampled row if seen again was suggested to us by an anonymous reviewer. Instead of using a separate exponential embedding to compute approximate $\ell_p$ sensitivities, the alternate algorithm uses the sampled matrix itself to compute sensitivities. We can analyze the algorithm using carefully defined martingales and show that the algorithm computes an $\ell_p$ subspace embedding with high probability. The alternate algorithm is simpler than Algorithm~\ref{alg:one-pass-arbitrary-order} but we show that a version of our Algorithm~\ref{alg:one-pass-arbitrary-order} that just outputs sensitivity estimates is adversarially robust (see Section~\ref{sec:adversarial}). Additionally our analysis of the limited independent exponential random variables to estimate $\ell_p$ norms in the stream makes progress towards answering the open question in Andoni \cite{andoni2017high}, and may be of independent interest. 

\begin{algorithm}
\KwIn{$n \in \Z$, Stream of elements $(a_1,t_1),\ldots,(a_n,t_n) \in \R^d \times [N]$}
\KwOut{Subspace embedding for $\dedup(A)$}
$M \gets \emptyset$\;
\For{$i = 1,\ldots,n$}{
    $\tau_i \gets \max_x {|\la a_i, x\ra|^p}/{\lp{Mx}^p}$\;
    $p_i \gets \min(1,\alpha \tau_i)$\;
    \If{$(a_i, t_i, *)$}{Delete $(a_i,t_i, *)$ from $M$\;}
    With probability $p_i$, add $(a_i,t_i, 1/p_i^{1/p})$ to $M$\;
}
\Return $M$\;
\caption{Alternate 1-pass Subspace Embedding}\label{alg:alternate-algorithm}
\end{algorithm}

==> bounded_entries.tex <==
While the subspace embedding construction in the previous section has to make $O(\log n)$ passes over the stream of updates to the matrix, or $t$ passes but at least $n^{1/t}$ memory, we show that if the $n \times d$ matrix $A$ has integer entries with absolute values bounded above by $\poly(d)$ (note $d \ll n$) and we only want to estimate $\lp{\dedup(A)x}^p$ for vectors $x$ with integer entries bounded by $\poly(d)$ as well, we show that there is a $1$-pass algorithm that constructs a data structure that can be stored using $\poly(d, \log n)/\varepsilon^2$ bits and lets us estimate $\lp{\dedup(A)x}^p$ up to a $1 \pm \varepsilon$ factor for any integer vector $x$ with coordinates bounded by $\poly(d)$.

The algorithm is again based on $\ell_0$ sampling and crucially uses the fact that given any such $x$, the nonzero coordinates of the vector $\dedup(A) x$ have values between $1$ and $\poly(d)$. By Hoeffding's inequality, uniformly sampling (with replacement) $\poly(d)^2\log(1/\delta)/\varepsilon^2$ non-zero coordinates of the vector $Ax$ lets us estimate $\lp{\dedup(A)x}^p$ up to $1 \pm \varepsilon$ factor for any constant $p$. We now show that there is a $1$-pass algorithm that constructs a data structure that lets us sample non-zero coordinates of the vector $\dedup(A) \cdot x$. Importantly, the algorithm needs no knowledge of $x$ while constructing the data structure.

Let $V$ be a $\poly(d)^d \times d$ matrix that contains a row for each possible $a \in \set{-\poly(d), \ldots, \poly(d)}^d$. At the end of the stream, $V$ is defined to be the matrix that satisfies the following property: $
    V_{i*} = \dec(i) \cdot \text{freq}_i
$
where $\text{freq}_i$ denotes the difference of the number of insert and delete requests for the row $\dec(i)$ in the stream. Let $\bL_{\text{count}} : \R^{\poly(d)^d} \rightarrow \R^{\ell}$ be the randomized linear map in Theorem~\ref{thm:count-approximation} with failure probability $\le \poly(d)^{-d}$ and accuracy $\varepsilon$ and let $\bL_{\text{sample}} : \R^{\poly(d)^d} \rightarrow \R^{\ell'}$ be the randomized linear map in Theorem~\ref{thm:l0-sample}. Clearly, the matrices $\bL_{\text{count}} \cdot V$ and $\bL_{\text{sample}} \cdot V$ can be computed in 1-pass in a stream. We store both these matrices $\bL_{\text{count}} \cdot V$ and $\bL_{\text{sample}} \cdot V$ after processing the stream.

Now consider a fixed vector $x \in \set{-\poly(d), \ldots, \poly(d)}^d$. Note that $(Vx)_{i} = \text{freq}_i \la \dec(i), x\ra$. Hence the $i$-th coordinate of $Vx$ is zero if $\text{freq}_i = 0$ or if $\dec(i) \perp x$. Thus the non-zero coordinates of $Vx$ exactly correspond to those coordinates of the vector $\dedup(A) \cdot x$ that are non-zero. Conditioned on non-failure of $\bL_{\text{count}}$ for the vector $Vx$, which happens with probability $\ge 1 - \poly(d)^{-d}$, we can estimate the number of non-zero coordinates of the vector $\dedup(A) \cdot x$ up to $1 \pm \varepsilon$ factor. Conditioned on the non-failure of $\bL_{\text{sample}}$ for the vector $Vx$, we can sample a uniform random non-zero coordinate from the vector $\dedup(A) \cdot x$. Thus if we use $O(\poly(d)/\varepsilon^2)$ independent copies of the randomized map $\bL_{\text{sample}}$, we can estimate $\lp{\dedup(A) \cdot x}^p$ up to $1 \pm \varepsilon$ factor with probability $\ge 1 - \poly(d)^{-d}$ by a union bound on the failure probabilities of $O(\poly(d)/\varepsilon^2)$ $\bL_{\text{sample}}$ maps, $\bL_{\text{count}}$ map and failure probability of the Hoeffding bound. Now we can union bound over the $\poly(d)^d$ possible vectors $x$ and obtain that we can estimate the $\lp{\dedup(A) \cdot x}^p$ for any $x \in \set{-\poly(d), \ldots, \poly(d)}^d$. The algorithm uses $O(\poly(d)/\varepsilon^2)$ bits of space.
\begin{theorem}
   For a constant $p>1$, given a stream ``insert/delete $a_1$'', \ldots, ``insert/delete $a_n$'' with $a_i \in \set{-M, \ldots, M}^d$ for $M = \poly(d)$, there is a streaming algorithm that makes a single passes over the requests that uses $\poly(d)/\varepsilon^2$ bits of space and outputs a data structure that can estimate $\lp{\dedup(A) \cdot x}^p$ up to $1 \pm \varepsilon$ factor for any $x \in \set{-M, \ldots, M}^d$. 
   \label{thm:bounded-entries-one-round}
\end{theorem}

==> deduplicated_embedding.tex <==
The following lemma lists some consequences of our $\ell_p \rightarrow \ell_{\infty}$ embedding and the partition result discussed in Section \ref{sec:tools}. We use this lemma to prove the correctness of our algorithm for the deduplicated matrix. Theorem~\ref{thm:partition-theorem} is used to prove that there is a \emph{small} set of prefixes of $A$ such that if the $\ell_p \rightarrow \ell_{\infty}$ embedding guarantee in Theorem~\ref{thm:lp-to-linf-embedding} holds for those prefixes, then it holds for all the prefixes of $A$. This lets us obtain an embedding guarantee with low distortion for all prefixes of $A$.
\begin{lemma}
\label{lma:upper-and-lower-bounds}
	Given an arbitrary matrix $A \in \R^{n \times d}$ with $\kappa^{\OL} := \kappa^{\OL}(A)$, there is a subset $P = \set{i_1,\ldots,i_r} \subseteq [n]$, $i_1 < \ldots < i_r$ of size $r = O((d\log n\kappa^{\OL})^{\max(p/2,1)}(d\log d + \log n))$ such that if $\bD$ is a random diagonal matrix constructed using an $O(d\log n + (p/2)(\log(d) + \log\log n +\log\log \kappa^{\OL}))$-wise independent hash family, then with probability $\ge 99/100$, all the following events hold:
	\begin{enumerate}
		\item If $i$ satisfies $i_j < i < i_{j+1}$, then for all $x$,
		\begin{align*}
			\lp{A_{1:i_j}x} \ge (1/4)\lp{A_{1:i}x}.
		\end{align*}
		\item For all $i$ and for all $x$,
		\begin{align*}
			\linf{\bD_{1:i}^{1/p}A_{1:i}x} &\ge \frac{\lp{A_{1:i}x}}{4C(d^3\log^4 n\log\log \kappa^{\OL})^{1/p}}\\
			\linf{\bD_{1:i}^{1/p}A_{1:i}x}&\le 4   Cd^{\max(1.5+1/p,0.5+3/p)}\poly(\log \kappa^{\OL}, \log n)\lp{A_{1:i}x}.
		\end{align*}
	\end{enumerate}
\end{lemma}

\subsection{Main Algorithm}\begin{algorithm}
\caption{Online $\ell_{\infty}$ Subspace Sketch Coreset \cite{woodruff2022high}}
\label{alg:l-infinity-coreset}
\DontPrintSemicolon	
\KwIn{$A\in \R^{n\times d}$}
\KwOut{Coreset $S \subseteq [n]$}
$S \gets \emptyset$\;
\For{$i \in [n]$}{
	\If{$\exists x \in \R^n : \la a_i, x\ra^2 \ge \opnorm{A|_S x}^2$}{
		$S \gets S \cup \set{i}$\;
	}
}
\Return{$S$}\;
\end{algorithm}
We use the deterministic algorithm (stated as Algorithm~\ref{alg:l-infinity-coreset} here) of \citet{woodruff2022high} to maintain an $\ell_\infty$ subspace embedding of $\bD_{1:i}A_{1:i}$ in the stream by computing a coreset. 

\begin{theorem}[{{\cite[Theorem~3.11]{woodruff2022high}}}]
	Let $A \in \R^{n \times d}$ be such that the sum of online leverage scores is bounded by 
	$
		\sum_{i=1}^n \tau_i^{\OL, \ell_2}(A) \le T
	$
	and let $S$ be the output of Algorithm~\ref{alg:l-infinity-coreset}. Then:
	
		(i) $|S| \le O(T)$ and (ii) $(1/\Delta)\linf{Ax} \le \linf{A|_{S}x}\le \linf{Ax}$ for all $x \in \R^d$ where $\Delta = O(\sqrt{T})$.
	
\end{theorem}

We now state our main result.
\begin{theorem}
	Given a matrix $A \in \R^{n \times d}$ along with tags as a stream of pairs of a row and a tag $(a_1, t_1),\ldots,(a_n,t_n)$ with $a_i \in \R^d$ and $t_i \in [N]$ for some $N \ge n$, let $B$ denote the matrix formed by rows corresponding to distinct tags in the stream. Algorithm~\ref{alg:one-pass-arbitrary-order} outputs a matrix $B'$ that with probability $\ge 9/10$ satisfies, for all vectors $x \in \R^d$, we have $\lp{B'x} = (1 \pm \varepsilon)\lp{Bx}$.
	
	The algorithm uses at most $O(d^{O(p)}\poly(\log(N), \log(\kappa^{\OL}(B)))/\varepsilon^2)$ bits of space with probability $\ge 99/100$.
	\label{thm:main-theorem}
\end{theorem}
\begin{algorithm}
\KwIn{$n \in \Z$, Stream of elements $(a_1, t_1),\ldots,(a_n,t_n) \in \R^d \times [N]$,  $\kappa^{\OL} \ge \kappa^{\OL}(\dedup(A)), p, \varepsilon$}	
\KwOut{Subspace Embedding for $\dedup(A)$}
\DontPrintSemicolon
$M \gets \emptyset$\;
Sample $\bh \sim H$ where $H = \set{h : [N] \rightarrow [N]}$ is $O(d\log n)$-wise independent hash family\;
\For{$i=1,\ldots,n$}{
	$\bD_{ii} \gets \bg(t_i)$ \tcp*{$\bg(t) = \min(\textnormal{round}(N/\bh(t)), n)$}
	Feed $\bD_{ii}^{1/p}a_i$ to the $\ell_\infty$ embedding and obtain $S_i\bD_{1:i}^{1/p}A_{1:i}$ \tcp*{Algorithm~\ref{alg:l-infinity-coreset}}
	$\zeta_i \gets \max_x \frac{|\la a_i, x\ra|^p}{\linf{S_i \bD_{1:i}^{1/p}A_{1:i}x}^p}$ \tcp*{Obtained by solving a convex optimization problem}
	$s_i \gets \zeta_i \cdot (C^pd^{\max(3p/2+2, p/2+4)}\poly(\log n, \log \kappa^{\OL}))$\;
	\If{$(a_i, t_i,*) \in M$}{
		Delete $(a_i,t_i,*)$ from $M$;
	}
	$p_i = \min(1, C\varepsilon^{-2}s_i d\log d)$\;
	Include $(a_i, t_i, p_i)$ into $M$ with probability $p_i$\;
}
\Return{matrix $B'$ with rows given by $(1/p_i^{1/p})a_i$ if $(a_i,t_i, p_i) \in M$}
\caption{1-pass Subspace Embedding\label{alg:one-pass-arbitrary-order}}
\end{algorithm}
\subsection{\texorpdfstring{$\ell_p$}{lp} Low Rank Approximation}
A simple consequence of being able to perform $\ell_p$ sensitivity sampling of the matrix $\dedup(A)$ is that the algorithm can be used to compute approximate solutions to the $\ell_p$ Low Rank Approximation problem \cite{robust-subspace-approximation} for constant $p$. They show that if $\bM$ is the $\ell_p$ sensitivity sampling matrix for $A\bR$ where $\bR$ is a sparse embedding matrix with $O(k)$ columns, then rows of the matrix $\bM A$ span a good rank $k$ $\ell_p$ low rank approximation for $\bM A$. Thus, running the sensitivity sampling algorithm on rows of the matrix $\dedup(A\bR)$ immediately gives us an approximate solution for the $\ell_p$ low rank approximation of $\dedup(A)$.

==> embedding_without_duplicates.tex <==
Given an $n \times d$ matrix, if the random diagonal matrix $\bD$ is constructed by defining $\bD_{ii} = 1/\bE_i$ where $\bE_1,\ldots,\bE_n$ are independent standard exponential random variables, then \citet{woodruff2013subspace} shows that with probability $\ge 9/10$, $\linf{\bD^{1/p} Ax}$ approximates $\lp{Ax}$ for all $x$ with low distortion. We extend their proof and show that a construction of $\bD$ using an $O(d\log n)$-wise independent hash family also linearly embeds the column space of $A$ into the $\ell_\infty$ space.

Assume that row $a_i$ of $A$ is tagged with $t_i \in [N]$ for some $N \ge n$ and assume without loss of generality that $N = 2^s$ and $n = 2^r$ for some $s \ge r$. Also assume that all the tags $(t_i)_{i \in [n]}$ are distinct. Let $H = \set{h : [N] \rightarrow [N]}$ be a $k$-wise independent hash family for some $k = O(d\log n + \log 1/\delta)$. Thus if $\bh \sim H$ is drawn uniformly at random, then the the random variables $\bh(t_1),\ldots,\bh(t_n)$ are $k$-wise independent. Define $\bg(t)$ as follows:
\begin{align}
\bg(t) :=  \min(\text{round}(N/\bh(t)), n),
\label{eqn:definition-of-g}
\end{align}
where $\text{round}(x)$ rounds $x$ to the largest integer $2^j \le x$. Hence, $\bg(t)$ takes values only in the set $\set{1 = 2^0, 2^1,\ldots, 2^r = n}$. We also have that the random variables $\bg(t_1),\ldots,\bg(t_n)$ are $k$-wise independent and for any $t$, for $q \in \set{0,1,\ldots,r-1}$, $\Pr[\bg(t) = 2^q] = 1/2^{q+1}$ and $\Pr[\bh(t) = 2^r=n] = 1/2^{r}$. 

Now define an $n \times n$ random diagonal matrix $\bD$ as follows: draw $\bh \sim H$ uniformly at random and let $\bD_{ii} = \bg(i)$.
%\subsection{Subspace Embeddings}

\begin{theorem}
Given $N = 2^r$	 and $n = 2^s$ for integers $r \ge s$, let $H = \set{h : [N] \rightarrow [N]}$ be an $O(d\log n + \log(1/\delta))$-wise independent hash family. If $\bh \sim H$ is a random hash function drawn from $H$ and a random diagonal matrix $\bD$ is constructed such that
\begin{align*}
    \bD_{ii} = \min(\textnormal{round}(N/\bh(i)), n),
\end{align*}
where $\textnormal{round}(x) = 2^{\floor{\log_2(x)}}$, for any given $n \times d$ matrix $A$, with probability $\ge 1 - \delta$, for all $x$,
\begin{align*}
   \linf{\bD^{1/p}Ax} &\ge \frac{\lp{Ax}}{2(C_2((d\log n)^3 + (\log 1/\delta)^3)\log n)^{1/p}}\\
   \text{and}\ \linf{\bD^{1/p}Ax}&\le \frac{d^{\max(1,1/2+1/p)}(\log n)^{1/p}}{\delta^{1/p}}\lp{Ax}.
\end{align*}
\label{thm:lp-to-linf-embedding}
\end{theorem}

==> frobenius_lra.tex <==
\textcolor{red}{Rewrite this section for general $\ell_p$ low rank approximation}
\begin{theorem}
	Given a matrix $A \in \R^{n \times d}$ along with tags as a stream of pairs of row and tag $(a_1, t_1),\ldots,(a_n,t_n)$, let $B$ denote the matrix formed by rows corresponding to distinct tags in the stream. Given a rank parameter $k$ and an accuracy parameter $\varepsilon$, there is an algorithm that outputs a $d \times k$ matrix $Q$ with orthonormal columns that with probability $\ge 9/10$ satisfies, for all vectors $x \in \R^d$,
	\begin{align*}
		\frnorm{B(I - Q\T{Q})} \le (1 + \varepsilon)\frnorm{B - [B]_k}.
	\end{align*}
	Further, the algorithm uses at most $d\poly(k, \log n, \log N, \log \kappa^{\OL}(B), 1/\varepsilon)$ space.
	\label{thm:main-low-rank-approximation}
\end{theorem}
\begin{proof}
Let $A \in \R^{n \times d}$ be an arbitrary matrix and let $\bG$ be a $d \times d'$ matrix of independent Gaussian entries drawn from $N(0,1/\sqrt{d'})$ for $d' = O(k/\varepsilon^2)$. \citet{cohen2015dimensionality} show that there exists $c$, such that with probability $\ge 99/100$, for any orthogonal projection matrix $P$ of rank $k$, we have
\begin{align*}
	(1-\varepsilon)\frnorm{(I-P)A}^2 \le \frnorm{(I-P)A\bG}^2 + c\le (1+\varepsilon)\frnorm{(I-P)A}^2.
\end{align*}
Now,
\begin{align*}
	\frnorm{(I - [A\bG]_k[A\bG]_k^+)A}^2 &\le \frac{\frnorm{(I-[A\bG]_k[A\bG]_k^+)A\bG}^2 + c}{1 - \varepsilon}\\
	&\le \frac{\frnorm{(I - [A]_k[A]_k^{+})A\bG}^2 + c}{1 - \varepsilon}\\
	&\le \frac{(1+\varepsilon)\frnorm{(I - [A]_k[A]_k^+)A}^2}{1-\varepsilon}\\
	&= (1 + O(\varepsilon))\frnorm{A - [A]_k}^2,
\end{align*}
which shows that column space of $A\bG$ spans a good rank $k$ approximation for the matrix $A$. As the matrix $[A\bG]_k[A\bG]_k^+A$ can be written as $A\bG Y$ for some rank $k$ matrix $Y$, we therefore have
\begin{align*}
	\min_{\text{rank-}k\, X}\frnorm{A\bG X - A}^2 \le (1+O(\varepsilon)) \frnorm{A - [A]_k}^2.
\end{align*}
Now the matrix $A\bG$ has $O(k/\varepsilon^2)$ columns. Let $A\bG = QR$ be the QR decomposition. Let $\bS$ be a random matrix constructed as follows: for each $i \in [n]$, with probability $p_i = \min(1, \alpha v_i)$ for some $v_i \ge \beta \tau_i^{\ell_2}(A\bG)$, include the row $1/\sqrt{p_i}e_i$ into the matrix $\bS$ i.e., $\bS$ is the sampling matrix corresponding to approximate $\ell_2$ sensitivities (leverage scores) of rows of $A\bG$. If $\alpha \ge \beta^{-1}\log(d)/\varepsilon^2$, then with probability $\ge 99/100$, for all $x$,
\begin{align*}
	\opnorm{\bS A\bG x} = (1 \pm \varepsilon)\opnorm{A\bG x}
\end{align*}
and hence for all $x$,
\begin{align*}
	\opnorm{\bS Qx} = (1 \pm \varepsilon)\opnorm{Qx}.
\end{align*}
Also note that by definition, $\tau_i^{\ell_2}(A\bG) = \opnorm{Q_{i*}}^2$. So the leverage score sampling matrix also corresponds to a ``squared length sampling'' matrix for $Q$ and hence for the pair $(Q,A)$, if $\alpha \ge \beta^{-1}/\varepsilon^2$, we have the following Approximate Matrix Multiplication guarantee:
\begin{align*}
	\frnorm{\T{Q}\T{\bS}\bS A - \T{Q}A} \le (\varepsilon/\sqrt{d'})\frnorm{Q}\frnorm{A}.
\end{align*}
Using Theorem~7.10 of \cite{cw12}, we obtain that $\bS$ is a weak affine embedding and satisfies for any matrix $X$,
\begin{align*}
	\frnorm{\bS(QX - A)}^2 - \frnorm{\bS\tilde{A}}^2 = (1 \pm 2\varepsilon)\frnorm{QX - A}^2 - \frnorm{\tilde{A}}^2,
\end{align*}
where $\tilde{A} = Q\T{Q}A - A$. Let $\tilde{X} := \argmin_{\text{rank-}k\, X}\frnorm{\bS (QX - A)}$ and let $X^* := \argmin_{\text{rank-}k\, X}\frnorm{QX - A}$. Now,
\begin{align*}
	\frnorm{Q\tilde{X} - A}^2 &\le \frac{\frnorm{\bS(Q\tilde{X} - A)}^2 - \frnorm{\bS \tilde{A}}^2 + \frnorm{\tilde{A}}^2}{1 - 2\varepsilon}\\
	&\le\frac{\frnorm{\bS(Q{X^*} - A)}^2 - \frnorm{\bS \tilde{A}}^2 + \frnorm{\tilde{A}}^2}{1 - 2\varepsilon}\\
	&\le \frac{(1+2\varepsilon)\frnorm{QX^* - A}^2 }{1-2\varepsilon}\\
	&\le (1 + O(\varepsilon))\frnorm{QX^* - A}^2\\
	&\le (1 + O(\varepsilon))\frnorm{A - [A]_k}^2.
\end{align*}
Thus solving $\min_{\text{rank-}k\, X}\frnorm{\bS A\bG X - \bS A}$ gives a matrix $\tilde{X}$ such that the rowspace of $\tilde{X}$, which has dimension $k$, is a $1+O(\varepsilon)$ approximation for the Frobenius norm low rank approximation problem.

We can implement this algorithm in $d\poly( k/\varepsilon, \log \kappa^{\OL}(\dedup(A\bG)), \log n, \log N)$ space for the deduplicated matrix by simply running the leverage score sampling algorithm (Algorithm~\ref{alg:one-pass-arbitrary-order}) on the matrix $\dedup(A\bG)$ and by storing the full row $a_i$ for each row sampled during the algorithm. At the end of the stream we can compute the optimal solution for the problem
\begin{align*}
    X^* = \argmin_{\text{rank-}k\, X}\frnorm{\bS \cdot \dedup(A\bG)X - \bS \cdot \dedup(A)}
\end{align*}
and then the $k$ dimensional rowspace is a $1+O(\varepsilon)$ approximation to the best rank $k$ subspace for rank $k$ approximation of $\dedup(A) = B$ in Frobenius norm. In Lemma~\ref{lma:bounding-kappa-AG}, we show that with high probability $\kappa^{\OL}(\bG) = O(d\kappa^{\OL}(A))$ and therefore, with high probability the algorithm only needs $d \poly(k/\varepsilon, \log \kappa^{\OL}(\dedup(A)), \log n, \log N)$ space.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> intro.tex <==
We study randomized numerical linear algebra problems when the rows of an $n \times d$ matrix $A$ are presented one at a time to an algorithm in an arbitrary order in a data stream. The algorithm is only allowed to make a few passes over the stream, and because of the large size of the input matrix $A$, can only afford to store a small summary or sketch of what it has seen at any point of time. A variety of linear algebraic problems have been studied in this model, including least squares and robust regression \cite{DBLP:conf/stoc/ClarksonW09,DBLP:conf/icml/CormodeDW18,woodruff2022high}, low rank approximation \cite{DBLP:conf/stoc/BoutsidisWZ16, DBLP:journals/siamcomp/GhashamiLPW16} and robust low rank approximation \cite{DBLP:conf/stoc/MahabadiRWZ20,DBLP:conf/icml/JiangLLMW21,DBLP:conf/nips/LevinSW18}, approximate matrix product \cite{DBLP:conf/stoc/ClarksonW09,DBLP:conf/icml/CormodeDW18}, and numerous other works and problems.

A notable omission in previous work is that of dealing with data with {\it duplicates}, e.g., rows of a matrix which may occur more than once. This is a common problem in the data stream model. For example, the same data record, corresponding to a distinct row, may be collected from multiple different sources, such as a person's cell phone and the same person's laptop, and placed together in the stream. Another example is when the stream is sent over a network and due to network failure the sender may send some pieces of the data multiple times. Other examples are when a tweet was retweeted by different users and repeated multiple times and to provide diversity we intend to avoid prioritizing duplicated celebrity tweets, or when we have files that are copied multiple times by several users and we intend to do a calculation over the space of the original files. Hence, in a number of cases, a row should be given the same importance as that of another row which occurs multiple times in the stream. 

With this motivation we would like to first remove the duplicates in a data preprocessing step, and then solve an optimization problem only on the set of {\it distinct} records. This is sometimes referred to as {\it entity resolution}, also called {\it data deduplication} or {\it record linkage}, see, e.g., \cite{DBLP:journals/pvldb/DongN09,DBLP:journals/tkde/ElmagarmidIV07,DBLP:books/daglib/0018313,DBLP:conf/sigmod/KoudasSS06}, but such methods do not apply in the data stream model in which we only have a small amount of memory and cannot store the entire set of distinct items explicitly. Deduplication is also especially important for public-private on-device model \cite{EEM19} and the centralized public-private model \cite{CEKL15}, where information is propagated along a graph, and statistics of the graph union (rather than the multigraph) are desired. For deduplication in the context of classification and other machine learning optimization problems see, e.g., \cite{mlEntity}. Another application is to perform regression and ridge regression on database joins \cite{DBLP:conf/pods/Khamis0NOS18,DBLP:conf/icml/JayaramSWY21}, where one may first wish to perform a SELECT DISTINCT on the join output before fitting a regression model.  
There are a few data stream algorithms that work even in the presence of duplicates. One such algorithm is that of outputting a random sample from the set of distinct data stream items, which is sometimes referred to as $F_0$-sampling or $\ell_0$-sampling  \cite{DBLP:journals/dpd/CormodeF14,cz18,FIS08,JST11,T15}. Other than sampling, norm estimation on the deduplicated stream was studied in the context of mining multigraph streams \cite{DBLP:conf/pods/CormodeM05}, where edges of a multi-graph could occur many times in the stream, but one may be interested in statistics of the underlying graph, which means that each edge should be counted only once. In \cite{DBLP:conf/pods/CormodeM05}, streaming algorithms for estimating $F_p$-moments, finding heavy hitters, and computing range sums of the degree distribution in the graph, rather than the multigraph, were developed. A number of applications of this framework were discussed, such as when the graph corresponds to traffic on an IP network, the web-graph, and even telephone call graphs. 

Despite the above work on data stream algorithms in the presence of duplicates for graph problems, to the best of our knowledge there is no such work for optimization problems, including the large body of problems in randomized numerical linear algebra discussed above. In this model, we think of each row of $A$ arriving with a tag, and rows with the same tag should only be counted once. Note that for regression problems, we can include the vector $b$ of labels as an extra column in $A$, so we will just think of being given the matrix $A$. Formally, let $(a_1,t_1),\ldots,(a_n,t_n)$ be the stream of pairs of rows and tags with $a_i \in \R^d$ and $t_i \in [N]$ observed in the stream. Assume that if $t_i = t_j$, then $a_i = a_j$. Let $A$ be an $n \times d$ matrix with its rows given by $a_i$ for $i \in [n]$. Let $T := \setbuilder{i}{\text{for all $j < i$, $t_j \ne t_i$}}$ denote the set of positions in the stream where a tag is seen for the first time. Let $B := A|_{T}$ be the $|T| \times d$ matrix formed by the rows $(a_i)_{i \in T}$. We also use the notation $\dedup(A)$ to denote the matrix obtained by removing duplicate rows corresponding to a tag. Then we would like to solve an optimization problem, such as computing a subspace embedding or a low rank approximation (LRA), on the matrix $B = \dedup(A)$. 

In the model which allows deletions as well, the stream is assumed to be of the form ``insert/delete $a_i$'' and we assume that for any row the delete requests are at most equal to the insert requests. The matrix $\dedup(A)$ is then defined to be the matrix formed by rows that have more insert requests than delete requests. Additionally we assume that the rows $a_i \in \set{-M, \ldots, M}^d$ for $M = \poly(n)$, i.e., that the rows have bounded integer coordinates which is standard in the data stream literature. We can additionally assume the presence of tags just as in the previous case without changing the algorithms by much but we present our algorithms without rows attached to tags.

\subsection{Notation}
For any positive integer $n$, we use $[n]$ to denote the set $\set{1,\ldots,n}$. For $a,b > 0$ and $0 < \varepsilon < 1$, we use $a = (1 \pm \varepsilon)b$ if $(1 - \varepsilon)b < a < (1+\varepsilon)b$.

For a vector $x \in \R^{n}$ and $p \ge 1$, $\lp{x}$ denotes the $\ell_p$ norm of $x$ defined as $(\sum_{i \in [n]} |x_i|^p)^{1/p}$. The $\ell_{\infty}$ norm of $x$, denoted by $\linf{x}$ is defined as $\max_{i \in [n]}|x_i|$. Given a point $a \in \R^d$ and a compact set $S \subseteq \R^d$, we define $d(a, S) \coloneqq \min_{s \in S}\opnorm{a - s}$ to be the minimum distance between $a$ and a point in $S$. Given an $n \times d$ matrix $A$, $\frnorm{A}$ denotes the Frobenius norm of matrix $A$ defined as $(\sum_{i,j} A_{i,j}^2)^{1/2}$ and $\opnorm{A}$ denotes the spectral (operator) norm. For $i \in [n]$, $A_{i*}$ denotes the $i$-th row of matrix $A$ and for $j \in [d]$, $A_{*j}$ denotes the $j$-th column of $A$. We also use $a_1,\ldots,a_n$ to refer to the rows of matrix $A$. We use the notation $A_{1:i}$ to denote the matrix formed by the first $i$ rows of $A$. We call such matrices \emph{prefixes} of $A$. For a subset $T \subseteq [n]$, we use $A|_{T}$ or $A_T$ (when the notation is not cumbersome) to denote the matrix formed by rows that correspond to indices in $T$. For an $n \times d$ matrix $A$, we use $A^+$ to denote the Moore-Penrose pseudoinverse of matrix $A$. Given a matrix $A$, we call a matrix $A'$ an $\varepsilon$ $\ell_p$ subspace embedding if for all $x$, $\lp{A'x}= (1 \pm \varepsilon)\lp{Ax}.$
The distortion of a subspace embedding is defined as \[(\max_x \lp{Ax}/\lp{A'x})/(\min_x \lp{Ax}/\lp{A'x}).\]

We typically use bold symbols such as $\bD, \bS, \bh, \ldots$ to emphasize that these objects are sampled from an appropriate distribution.


\subsection{Our Results}
We prove that an $\ell_p$ subspace embedding for $\dedup(A)$ can be computed in a stream using $d^{O(p)}\poly(\log n, \log \kappa^{\OL}(\dedup(A)), \log N)/\epsilon^2$ space. Here $\kappa^{\OL}(\cdot)$ is defined as
\begin{align*}
    \kappa^{\OL}(M) := \frac{\opnorm{M}}{\min_i \sigma_{\min}(M_{1:i})},
\end{align*}
where $\sigma_{\min}(\cdot)$ denotes the smallest nonzero singular value of a matrix. For a matrix $M$ with integer entries with absolute values bounded above by $\poly(n)$, we have that $\kappa^{\OL}(M) \le (\poly(n))^d$ (see \cite[Lemma~37]{DBLP:conf/stoc/BoutsidisWZ16}).
\begin{theorem}[Informal, Theorem~\ref{thm:main-theorem}]
	Given a matrix $A \in \R^{n \times d}$ along with tags as an insertion-only stream of pairs of a row and a tag $(a_1, t_1),\ldots,(a_n,t_n)$ with $a_i \in \R^d$ and $t_i \in [N]$,  Algorithm~\ref{alg:one-pass-arbitrary-order} outputs a matrix $B'$ that with probability $\ge 9/10$ satisfies, for all vectors $x \in \R^d$,
	$
		\lp{B'x} = (1 \pm \varepsilon)\lp{\dedup(A) x}.
	$
	Further, the algorithm uses at most \[O(d^{O(p)}\poly(\log n, \log \kappa^{\OL}(\dedup(A)), \log N)/\varepsilon^2)\] space with probability $\ge 99/100$.
\end{theorem}
We do not focus on optimizing the exponent of $d$ in the above algorithm. It may be possible to obtain a better dependence on $p$ in the exponent of $d$ by using $\ell_p$ Lewis weight sampling \cite{cohen2015lp} and a better dependence on $\kappa^{\OL}$ using results from \cite{woodruff2022high}. 

Using this result, we obtain small-space approximate algorithms for $\ell_p$ low rank approximation.
\begin{theorem}[Informal]
    Given an insertion-only stream of pairs of a row and a tag and a constant $p > 1$, there is an algorithm that uses $O(d \cdot k^{O(p)} \poly(\log n, \log \kappa^{\OL}(\dedup(A\bR)), \log N))$ bits of space and outputs a $k$ dimensional subspace $V'$ that satisfies
    \begin{align*}
        \sum_{a \in \dedup(A)} d(a, V')^p \le \poly(k)\min_{\text{$k$ dim $V$}}\sum_{a \in \dedup(A)}d(a, V)^p.
    \end{align*}
    Here $\bR$ is a sparse random matrix as in Theorem~32 of \cite{robust-subspace-approximation}.
\end{theorem}

We then give a different \emph{deterministic} algorithm to solve the $p=\infty$ version of the above problem.
\begin{theorem}[Informal, Theorem~\ref{thm:max-distance-to-a-subspace}]
    Given an insertion-only stream of pairs of a row and a tag, there is a \emph{deterministic} algorithm that uses
    $d \cdot k \poly(\log \kappa^{\OL, k}(\dedup(A)), \log n )$ bits of space and produces a rank $k$ subspace $V'$ that satisfies,
    \begin{align*}
        \max_{a \in \dedup(A)} d(a, V') \le \Delta \min_{\text{$k$ dim $V$}}\max_{a \in \dedup(A)} d(a, V)
    \end{align*}
    where $\Delta = \sqrt{k}\poly(\log n, \log \kappa^{\OL, k}(\dedup(A)))$. Here  $\kappa^{\OL, k}(\cdot)$ denotes the rank $k$ online condition number that we define later.
\end{theorem}
For streams with deletions as well, we given an $O(\log n)$ pass algorithm to construct an $\ell_p$ subspace embedding.
\begin{theorem}[Informal, Theorem~\ref{thm:logn-round-subspace-embedding}]
    For a constant $p>1$, given a stream of $n$ insert and delete requests for rows in $\set{-M, \ldots, M}^d$ for $M = \poly(n)$, there is an algorithm that makes $O(\log n)$ passes over the stream and uses $\poly(d, \log n)$ bits of space and computes a $1 \pm \varepsilon$ $\ell_p$ subspace embedding for the matrix $\dedup(A)$.
\end{theorem}
A version of the algorithm that that samples $n^{1/t}$ fraction of rows at each level needs only $O(t)$ rounds and uses $O(n^{1/t}\poly(d, \log n))$ bits of space giving a smooth tradeoff.

The above algorithm uses only a small amount of space but takes $O(\log n)$ passes which may be  infeasible to implement in the context of network streams etc. We show that by making stronger assumptions on entries of the rows and on the entries of the vectors $x$ for which we want to approximate $\lp{\dedup(A) \cdot x}^p$, there is a $1$-pass algorithm that computes a data structure that lets us approximately compute $\lp{\dedup(A) \cdot x}^p$ for all such $x$.
\begin{theorem}[Informal, Theorem~\ref{thm:bounded-entries-one-round}]
    For a constant $p > 1$, given a stream of $n$ add and delete requests for rows in $\set{-M, \ldots, M}^d$ for $M = \poly(d)$, there is a $1$-pass algorithm that uses $\poly(d, \log n)\varepsilon^{-2}$ bits of space and outputs a data structure that with probability $\ge 99/100$ lets us approximate $\lp{Ax}^p$ for any $x \in \set{-M,\ldots,M}^d$.
\end{theorem}


% To obtain $o(n)$ space in the above results, we first show that $O(d\log(n))$-wise independent hash functions are sufficient to obtain an $\ell_p \rightarrow \ell_{\infty}$ embedding for a $d$ dimensional subspace of $\R^n$. This is an improvement over the earlier construction of an $\ell_p \rightarrow \ell_\infty$ embedding by \cite{woodruff2013subspace} which requires independent exponential random variables. \citet{andoni2017high} conjectured that $O(\log n)$-wise independent random variables are sufficient to approximate the $\ell_p$ norm of a vector up to a constant factor in a turnstile stream. With the following result, we make progress towards proving the conjecture and show that $O(\log n)$-wise independent random variables are indeed sufficient to approximate the $\ell_p$ norm of a vector up to $\poly(\log n)$ factors.
% \begin{theorem}[Informal]
% Given $n = 2^s$ for an integer $s$, let $H = \set{h : [n] \rightarrow [n]}$ be an $O(d\log n)$-wise independent hash family. If $\bh \sim H$ is a random hash function drawn from $H$ and a random diagonal matrix $\bD$ is constructed such that
% \begin{align*}
%     \bD_{ii} = \textnormal{round}(n/\bh(i)),
% \end{align*}
% where $\textnormal{round}(x) = 2^{\floor{\log_2(x)}}$, for any given $n \times d$ matrix $A$, with probability $\ge 99/100$,
% \begin{align*}
%     \frac{\lp{Ax}}{C(d^3\log^4 n)^{1/p}} \le \linf{\bD^{1/p}Ax} \le {d^{\max(1,1/2+1/p)}(\log n)^{1/p}}\lp{Ax}.
% \end{align*}
% \end{theorem}
% See the full theorem statement for failure probability dependent distortion bounds for our $\ell_p \rightarrow \ell_{\infty}$ embedding. 

\input{overview}

\subsection{Preliminaries}\label{sec:prelims}
\input{prelims}

==> lower_bounds.tex <==
\subsection{Determinstic Streaming Algorithms}
The $\ell_p$ sensitivity sampling algorithm shows that given any $n \times d$ matrix $A$, there is a subset $S \subseteq [n]$ of size $O(d^{\max(p/2+1,2)}\log d/\varepsilon^2)$ such that the rows of $A_S$ appropriately scaled gives an $\ell_p$ subspace embedding for the matrix $A$. This immediately implies a deterministic streaming algorithm that uses $\poly(d, 1/\varepsilon, \log n)$ space and outputs an $\ell_p$ subspace embedding for the matrix $A$ in the row arrival model using the merge-and-reduce framework whereby the streaming algorithm stores an $\ell_p$ embedding for the matrix seen until now using $\poly(d, 1/\varepsilon, \log n)$ space, processes and stores the next $\poly(d,1/\varepsilon,\log n)$ rows, and then reduces the matrix formed by the $\ell_p$ subspace embedding and the new rows by computing a new $\ell_p$ subspace embedding using a deterministic algorithm. The deterministic algorithm just na\"ively enumerates over all subsets and reweightings of the rows and finds an $\ell_p$ subspace embedding. Clearly, this deterministic algorithm, using $\poly(d,1/\varepsilon,\log n)$ space, outputs an $\ell_p$ subspace embedding for the matrix $A$ at the end of the stream.

But we can show that any deterministic streaming algorithm that produces an $\ell_p$ subspace embedding for the deduplicated matrix must use $\Omega(n)$ space. We show this lower bound by reducing from the Equal-vs-Spread problem. \citet{chakrabarti2016strong} give a communication lower bound for the $t$ player version of this problem.
\begin{theorem}
    Any deterministic streaming algorithm that streams a matrix $A$ in the row arrival model and computes an $\ell_p$ subspace embedding of distortion $C$ for the matrix $\dedup(A)$ must use $\Omega(n/C^{2p} - p\log C)$ bits of space.
    \label{thm:lower-bound-deterministic-algorithms}
\end{theorem}
\subsection{Sketching Algorithms}
By reducing from the $t$-player set Disjointness problem, we can show lower bounds on the sketch size required to compute a subspace embedding for the deduplicated matrix. Note that the lower bounds here are when there are no tags available and deduplication happens by removing rows that are equal irrespective of tags.

In the multiparty set-disjointness problem, each of the $d$ players is given a subset of $[n]$ with the promise that either the subsets received by all the players are mutually disjoint or there is one unique element present in all the sets that are otherwise disjoint. In the blackboard communication model, where each message sent by a player is seen by all other players, it is shown that this problem has a randomized lower bound of $\Omega(n/d)$ bits \cite{gronemeier2009asymptotically, jayram2009hellinger}. 

\begin{theorem}
    If $\bS$ is a random sketching matrix, with entries of bounded precision, such that for all matrices $A$, an $\ell_p$ subspace with distortion $C < d^{1/2-1/2p}$ can be computed using $\bS A$ with probability $\ge 9/10$, then the sketching matrix $\bS$ must have $\tilde{\Omega}(n/d^2)$ rows.
    \label{thm:lower-bounds-sketching-algorithms}
\end{theorem}

==> overview.tex <==
\subsection{Technical Overview}
\paragraph{Sensitivity Sampling} Given a matrix $A$, let \[\tau_i^{\ell_p}(A) \coloneqq \max_x {|\la a_i, x\ra|^p}/{\lp{Ax}^p}\] be the $\ell_p$ sensitivity of row $i$. Note that $\ell_2$ sensitivities are also called \emph{leverage scores}. If each row $a_i$ of $A$ is sampled with probability $p_i = \min(1, \alpha\tau_i^{\ell_p}(A))$, and if sampled, then the row $a_i/p_i^{1/p}$ is included in a matrix $A'$, then we can show that with probability $\ge 1 - \delta$, for all vectors $x \in \R^d$, $
	\lp{A'x} = (1 \pm \varepsilon)\lp{Ax}
$
if $\alpha = \Omega(\varepsilon^{-2}(d\log(d) + \log(1/\delta)))$. The sampling process is called \emph{sensitivity sampling} and has previously been used in \cite{dasgupta2009sampling} to obtain fast algorithms for $\ell_p$ linear regression and for computing $\ell_1$ subspace embeddings (see \cite{woodruff2014sketching}). We can bound the sum of $\ell_p$ sensitivities by $O(d^{\max(p/2, 1)})$ and hence the above sensitivity sampling procedure samples at most $O(\varepsilon^{-2}d^{\max(p/2,1)}(d\log d + \log(1/\delta)))$ rows with high probability. 

When operating in a stream, as the $\ell_p$ sensitivities cannot be computed, we instead use \emph{online} sensitivities defined by $\tau_i^{\OL,\ell_p}(A) \coloneqq \max_x |\la a_i, x\ra|^p/\lp{A_{1:i}x}^p$, where $A_{1:i}$ is the $i \times d$ matrix formed by the first $i$ rows in the stream. Note that for all $i$, online sensitivities are at least \emph{offline} sensitivities. As the sensitivity sampling algorithm only needs upper bounds on offline sensitivities, the sampling process using online sensitivities also produces a subspace embedding. Moreover, for ``well-conditioned'' $A$, we can show that the sum of online sensitivities is comparable to the sum of offline sensitivities. We prove this by extending the ideas from \cite{cohen2016online,braverman2020near}. To bound the sum of online sensitivities, we define a condition number parameter $\kappa^{\OL}$ for matrix $A$ as follows:
\begin{align*}
	\kappa^{\OL}(A) = \frac{\opnorm{A}}{\min_i \sigma_{\min}(A_{1:i})},
\end{align*}
where $\sigma_{\min}(\cdot)$ denotes the smallest nonzero singular value of a matrix and show that sum of online $\ell_p$ sensitivities of a matrix $A$ is bounded by $O((d \log n\kappa^{\OL}(A))^{\max(p/2,1)}\log n)$.

\paragraph{A Subspace Embedding for the Deduplicated Matrix} Our algorithm implements the above  online $\ell_p$ sensitivity sampling algorithm on the deduplicated matrix. Given a row $a_i$, we need to be able to compute $\max_x |\la a_i, x\ra|^p/\lp{\dedup(A_{1:i})x}^p$. Crucially, if the row $a_i$ was previously seen and sampled at that time, we delete that sample so that we give only \emph{one} copy of a row a chance to be sampled in the final output. The other thing that remains is to be able to estimate $\lp{\dedup(A_{1:i})x}^p$ for any $x$. For this we use exponential random variables to embed $\ell_p$ to $\ell_{\infty}$ while using the same exponential random variable for each copy of a row. The fact that exponential random variables can be used to embed $\ell_p$ to $\ell_{\infty}$ was used in \cite{woodruff2013subspace}. One of our main contributions is showing that exponential random variables generated using only limited independence also suffices for this purpose. This is important in the streaming setting as we need to be able to generate the same exponential random variable each time we see a copy of a row and storing all the previously used exponential random variables is infeasible as it may require a linear amount of memory. Note that the usual derandomization of streaming algorithms using Nisan's PRG does not apply here as our algorithm is non-linear and the stream cannot be rearranged to make the usual argument go through. We show that the $\ell_p$ sensitivity sampling algorithm immediately extends to give approximate solutions for the $\ell_p$ Low Rank Approximation \cite{deshpande2007sampling,deshpande2011algorithms} using results from \cite{robust-subspace-approximation}. We further show that a version of our algorithm can be used to output approximations to $\ell_p$ sensitivities of the rows in the stream with respect to the deduplicated matrix and show that the algorithm is robust to adversaries. The robust algorithm only incurs a polynomial factor overhead in space. Our algorithm is inspired by the sketch-switching technique of \cite{ben2022framework}. 

% \paragraph{Subspace Embedding for Deduplicated Matrix} Recall our setting: let $(a_1,t_1),\ldots,(a_n,t_n)$ be the stream of pairs of rows and tags with $a_i \in \R^d$ and $t_i \in [N]$ observed in the stream. Assume that if $t_i = t_j$, then $a_i = a_j$. Let $A$ be an $n \times d$ matrix with its rows given by $a_i$ for $i \in [n]$. Let $T := \setbuilder{i}{\text{for all $j < i$, $t_j \ne t_i$}}$ denote the set of positions in the stream where a tag is seen for the first time. Let $B := A|_{T}$ be the $|T| \times d$ matrix formed by the rows $(a_i)_{i \in T}$. We also use the notation $\dedup(A)$ to denote the matrix obtained by removing duplicate rows corresponding to a tag.

% Now consider the following algorithm for computing a subspace embedding for the deduplicated matrix. Let the algorithm maintain a set $M = \set{(a_j,t_j,p_j),\ldots}$ of the rows it has previously sampled. Let $(a_i, t_i)$ be the row that is currently being processed. In the first step, if there is an entry $(a_i,t_i, *)$ already present in $M$, then delete the entry. Next suppose we can compute 
% \begin{align}
%  \tau_i := \max |\la a_i, x\ra|^p/\lp{\dedup(A_{1:i})x}^p   
%  \label{eqn:overview:tau-definition}
% \end{align}
% i.e., the sensitivity of $a_i$ with respect to the ``deduplicated matrix'' seen till now in the stream. Note that $\tau_i \ge \tau_i^{\ell_p}(\dedup(A)) := \max_x |\angles{a_i, x}|^p/\lp{\dedup(A)x}^p$. Let $p_i := \min(1, \alpha \tau_i)$ be the sampling probability. Now, with probability $p_i$, include the entry $(a_i, t_i, p_i)$ into the set $M$. Then move to processing the $(i+1)$-th element in the stream. Consider $M$ at the end of processing the stream. The deletion step ensures that only rows that correspond to last occurrence of a tag in the stream are given a chance to be in the set $M$. And for the last occurrence $(a_i,t_i)$, the value of $\tau_i$ computed is at least $\max_x |\la a_i, x\ra|^p/\lp{\dedup(A)x}^p$ i.e., the offline $\ell_p$ sensitivity of $a_i$ with respect to the deduplicated matrix. Hence, this algorithm simulates the $\ell_p$ sensitivity sampling algorithm on the deduplicated matrix and therefore an appropriate matrix constructed from the set $M$ at the end of the stream will be a subspace embedding for $\dedup(A)$ with large probability. The main obstacle in implementing the algorithm is to compute $\tau_i$ as defined or an approximation for $\tau_i$ when processing the $i$-th element in the stream.

% Our main starting point for handling deduplicated instances is the observation that we can linearly embed an $\ell_p$ subspace into an $\ell_{\infty}$ subspace by scaling each coordinate with an appropriate function of independent exponential random variables. The property of interest is called ``max-stability'' of standard exponential random variables and states that for $\lambda_1,\ldots,\lambda_n > 0$, the random variable $\max(\lambda_1/\bE_1,\lambda_2/\bE_2,\ldots,\lambda_n/\bE_n)$ is distributed as $(\sum_i \lambda_i)/\bE$ if $\bE_1,\ldots,\bE_n$ are independent standard exponential random variables with $\bE$ also being a standard exponential random variable. Max-stability property implies that if $\bD$ is a random diagonal matrix such that $\bD_{ii} = 1/\bE_{i}$, then for any $x$, $\linf{\bD^{1/p} x}^p$ is distributed as $\lp{x}^p/\bE$. This observation was used to approximate $\ell_p$ norm of a vector in turnstile streams by \citet{andoni2017high} and later extended by \citet{woodruff2013subspace} to construct $\ell_p \rightarrow \ell_\infty$ subspace embeddings with low distortion for $d$-dimensional subspaces and show that for all vectors $x$, $\linf{\bD^{1/p} Ax} \approx \lp{Ax}$ up to $\poly(d)$ factors.

% Recall that our aim is to compute $\tau_i$ defined in \eqref{eqn:overview:tau-definition} after seeing $i$-th item in the stream. The advantage with $\ell_\infty$ norm in handling duplicates is the following. Suppose $x_1 = x_2$ and instead of generating exponential random variables $\bE_1,\ldots,\bE_n$ independently, we set $\bE_1 = \bE_2$. Then we have
% \begin{align*}
% 	\linf{(x_1/\bE_1^{1/p},x_2/\bE_2^{1/p},\ldots,x_n/\bE_n^{1/p})}^p = \linf{(x_2/\bE_2^{1/p},\ldots,x_n/\bE_n^{1/p})}^p \equiv (\sum_{i=2}^n x_i^p)/\bE.
% \end{align*}
% The above equality holds as removing duplicate coordinates does not affect the $\ell_{\infty}$ norm of a vector. Thus, if the matrix $\bD$ is generated as described above with a modification that if $t_i = t_j$, then $\bE_i = \bE_j$ instead of using a fresh exponential random variable, then we have that for any $x$,
% \begin{align*}
%     \linf{\bD^{1/p}Ax} = \linf{\bD^{1/p}|_T\, \dedup(A)x}
% \end{align*}
% and then using the embedding result of \cite{woodruff2013subspace}, we obtain that for all $x$, $\linf{\bD^{1/p}|_T\, \dedup(A)x} \approx \lp{\dedup(A) x}$ which is exactly what we need to compute in the stream to compute $\tau_i$.

% Earlier construction of $\ell_p \rightarrow \ell_\infty$ embedding \cite{woodruff2013subspace} uses independent exponential random variables. But as discussed above, we need to generate an identical random variable if a tag that has previously been seen in the stream appears again. Storing the mapping of tags to corresponding exponential random variables in the stream is infeasible as it requires $\Theta(n)$ memory. We solve this problem by instead using an $O(d\log n)$-wise independent hash family and replacing the exponential random variable with a discrete random variable that takes values in the set $\set{2^0,2^1,2^2,2^3,\ldots,2^{\log(n)}}$. For simplicity, assume that $n$ is a power of $2$, the tags are all from the set $[n]$ and that $H = \set{h : [n] \rightarrow [n]}$ is an $O(d\log n)$-wise independent hash family. Let $\bh \sim H$ be a uniformly random hash function drawn from $H$. We show that if the $n \times n$ matrix $\bD$ is generated as
% \begin{align*}
%     \bD_{ii} = \text{round}(n/\bh(i)),
% \end{align*}
% where $\text{round($x$)} = 2^{\floor{\log_2(x)}}$, then with high probability, for all $x$, $\linf{\bD^{1/p}Ax} \approx \lp{Ax}$. Concretely, we show that if $H$ is an $O(d\log n + \log 1/\delta)$-wise independent hash family, then with probability $\ge 1 - \delta$, for all $x \in \R^d$,
% \begin{align}
%     \frac{\lp{Ax}}{2(C_2((d\log n)^3 + (\log 1/\delta)^3)\log n)^{1/p}} \le \linf{\bD^{1/p}Ax} \le \frac{d^{\max(1,1/2+1/p)}(\log n)^{1/p}}{\delta^{1/p}}\lp{Ax}.
%     \label{eqn:overview:distortion-bound}
% \end{align}
% If we now instead define $\bD_{ii} = \text{round}(n/\bh(t_i))$, which ensures that all copies  of a row are scaled with the same random variable, we obtain $\linf{\bD^{1/p}Ax} = \linf{\bD^{1/p}|_{T}\, \dedup(A)x}$ and therefore that with probability $\ge 1 - \delta$, for all $x \in \R^d$,
% \begin{align}
%     \frac{\lp{\dedup(A)x}}{2(C_2((d\log n)^3 + (\log 1/\delta)^3)\log n)^{1/p}} \le \linf{\bD^{1/p}Ax} \le \frac{d^{\max(1,1/2+1/p)}(\log n)^{1/p}}{\delta^{1/p}}\lp{\dedup(A)x}.
%     \label{eqn:overview:failure-dependent-distortion}
% \end{align}

% Thus, to approximate $\tau_i = \max_x |\angles{a_i, x}|^p/\lp{\dedup(A_{1:i})x}^p$ defined previously, we only have to be able to compute $\linf{(\bD^{1/p} A)_{1:i}x}$ for all $x$. Unfortunately, we \emph{cannot} union bound over all $i \in [n]$ and claim that for all $i \in [n]$ and for all $x$,
% \begin{align*}
% 	\frac{\lp{\dedup(A_{1:i})x}}{2(C_2((d\log n)^3 + (\log 1/\delta)^3)\log n)^{1/p}} \le \linf{(\bD^{1/p} A)_{1:i}x}  \le \frac{d^{\max(1,1/2+1/p)}(\log n)^{1/p}}{\delta^{1/p}}\lp{\dedup(A_{1:i})x}
% \end{align*}
% as the required success probability of $1-\Theta(1/n)$ for the union bound to work makes the distortion of the embedding in \eqref{eqn:overview:failure-dependent-distortion} too large. We instead use a nice consequence of online leverage score sampling which lets us union bound over only $\poly(d,\log n, \log\kappa^{\OL})$ prefixes instead of all at $n$ prefixes. We now describe how to prove the existence of a nice set of prefixes.

% Given an arbitrary $n \times d$ matrix $A$, consider a run of online leverage score sampling of the rows of $A$. As described previously, if the probability of sampling row $i$ is $p_i := \min(1, \alpha \tau_i^{\OL,\ell_p}(A))$, for $\alpha = \Omega(d\log d + \log n)$, then with probability $\ge 1 - 1/\poly(n)$, the matrix computed by leverage score sampling algorithm is a $1/2$ $\ell_p$ subspace embedding for $A$. Moreover, the matrix computed after processing $n$ rows has at most $O(\sum_{i \in [n]}\tau_i^{\OL,\ell_p}(A)(d\log d + \log n))$ rows with high probability. Let $M_i$ be the matrix constructed by the algorithm after processing $i$-th row of $A$. By a union bound, we have with probability $\ge 1 - 1/\poly(n)$ that for all $i \in [n]$ and for all $x$,
% \begin{align*}
% 	\frac{1}{2}\lp{A_{1:i}x} \le \lp{M_i x} \le 2\lp{A_{1:i}x}.
% \end{align*}
% Now consider the set $P = \setbuilder{i}{M_i \ne M_{i-1}} \cup \set{n} = \set{i_1,\ldots,i_m}$ with $i_1 < i_2 < \ldots < i_m$. Condition on the event, which has a $1-1/\poly(n)$ success probability, that $M_n$ has $O(\sum_i \tau_i^{\OL,\ell_p}(A)(d\log d + \log n))$ rows and that for all $i \in [n]$, $M_i$ is an $\ell_p$ subspace embedding for $A_{1:i}$. Now, $|P| = O(\sum_{i\in [n]}\tau_i^{\OL,\ell_p}(A)(d\log d + \log n))$ and if $i \in [n]$ is such that $i_j < i < i_{j+1}$, then for all $x$,
% \begin{align*}
% 	\lp{A_{1:i} x} \le 2\lp{M_i x} = 2\lp{M_{i_j}x} \le 4\lp{A_{1:i_j}x},
% \end{align*}
% where the equality follows from the fact that $M_i = M_{i_j}$. Thus, there exists a small set of prefixes $(A_{1:i_j})_{i_j \in P}$ such that for all other prefixes $A_{1:i}$ there exists an $i_j \in P$ satisfying for all $x \in \R^d$,
% \begin{align*}
% 	\lp{A_{1:i_j}x} \le \lp{A_{1:i} x} \le 4\lp{A_{1:i_j}x}.
% \end{align*}
% For the matrix $B = \dedup(A)$, we consider such a set of prefixes $P$ and condition on the event that the corresponding prefixes of the random matrix $\bD^{1/p}|_T$ linearly embed prefixes of $B$ in $P$. As there are at most  
% \[O(\sum_{i\in [|T|]}\tau_i^{\OL,\ell_p}(B)(d\log d + \log n)) = O\left(\sum_{i \in [|T|]} \max_x\frac{|\angles{b_i,x}|^p}{\lp{B_{1:i}x}^p}(d\log d+ \log n)\right)\] 
% prefixes, we can union bound over $\bD|_T$ embedding all the prefixes in $P$ with low distortion using \eqref{eqn:overview:failure-dependent-distortion}. Conditioning on this event, we then show that good approximations for online sensitivities of \emph{all} rows of $\dedup(A)$ can be computed in the stream which finishes our proof. 

% \paragraph{Low Rank Approximation}
% Using the $\ell_p$ sensitivity sampling algorithm we described for computing an $\ell_p$ subspace embedding for $\dedup(A)$, we give an algorithm for finding a rank $k$ approximation for the matrix $\dedup(A)$ in Frobenius norm using $d \cdot \poly(k, \log \kappa^{\OL}(\dedup(A)), \log n, \log N)$ space. Our algorithm outputs a $d \times k$ matrix $Q$ with $k$ orthonormal columns such that
% \begin{align*}
%     \frnorm{\dedup(A) \cdot (I - Q\T{Q})} \le (1+\varepsilon)\frnorm{\dedup(A) - [\dedup(A)]_k},
% \end{align*}
% where $[\cdot]_k$ denotes the best rank $k$ approximation of a matrix in Frobenius norm.
% We use Projection Cost Preserving sketches  \cite{cohen2015dimensionality} and affine embeddings \cite{cw12} to reduce the low rank approximation problem to performing $\ell_2$ sensitivity sampling on $\dedup(A\bG)$ where $\bG$ is a Gaussian Random matrix with $O(k/\varepsilon^2)$ columns and then use our $\ell_p$ sensitivity sampling algorithm for deduplicated matrices for $p=2$. Similar techniques can be used to obtain bicriteria approximate solutions for rank $k$ approximation of $\dedup(A)$ in the sum-of-distances metric. This algorithm requires performing $\ell_1$ sensitivity sampling on the matrix $\dedup(A\bG)$ (see \cite[Theorem~4.1]{feng2021dimensionality}). 


\paragraph{A Coreset for $\ell_{\infty}$ Low Rank Approximation} Suppose we want to find a rank $k$ subspace that minimizes the maximum distance of a row in the input to the subspace. Note that this problem as already insensitive to duplicates. Consider the following simple algorithm in a stream: the algorithm maintains a set $S$ which is initialized to $\emptyset$. When processing the $i$-th row $a_i$, if there exists a rank $k$ projection matrix $P$ satisfying $\opnorm{\T{a_i}(I-P)} \ge \frnorm{A_S(I-P)}$, then modifies $S$ to $S \cup i$. We show that for ``well-conditioned'' instances, the set $S$ only has a few rows and that $A_S$ can be used to obtain a multiplicative approximation to the $\ell_{\infty}$ Low Rank Approximation problem.

\paragraph{Lower bounds for Deterministic algorithms and Sketching matrices} We show, by reductions from communication complexity problems, that any deterministic streaming algorithm that computes an $\ell_p$ subspace embedding of distortion $C$ for $\dedup(A)$ must use $\Omega(n/C^{2p} - p\log(C))$ bits and that any random linear sketching matrix $\bS$ such that $\bS A$ can be used to compute an $\ell_p$ subspace embedding of distortion $< d^{1-1/p}$ for $\dedup(A)$ must have $\tilde{\Omega}(n/d^2)$ rows. These lower bounds suggest that the randomization and row-arrival model we consider may be essential to obtain small space algorithms for computing $\ell_p$ subspace embeddings for deduplicated matrices.

\paragraph{Streams with Deletions} The algorithms we described critically use that the streams are insertion-only. When the streams are allowed to delete previously seen copies of rows, it is not clear how these algorithms can be modified to work. We give an $O(\log n)$-pass streaming algorithm that uses $\ell_0$-estimation and $\ell_0$-sampling algorithms from \cite{kane2010optimal,JST11} that can be used to estimate the number elements in a stream with non-zero frequency and sample a uniform random element with a non-zero frequency in the stream respectively. The algorithms provide us a primitive to sample uniformly random rows from the deduplicated matrix given a stream of rows with deletions. We show that these primitives are sufficient to implement a recursive $\ell_p$ sensitivity sampling algorithm to compute an $\ell_p$ subspace embedding. The offline (non-streaming) version of the $\ell_p$ sensitivity sampling algorithm was earlier used in \cite{cohen2015uniform, cohen2015lp}.


==> partition.tex <==
We prove that if a matrix $A \in \R^{n \times d}$ is ``well-conditioned'' the $\ell_p$ norm of products of prefixes of $A$ with a vector $x$ changes slowly. We show that there is a set $P \subseteq [n]$ of indices $\set{i_1,\ldots,i_r}$ for a small $r$ such that if $i_j \le i < i_{j+1}$, then for all $x$,
$
    \lp{A_{1:i_j}x} \le \lp{A_{1:i}x} \le 4\lp{A_{1:i_j}x}.
$
The statement shows that for a well-conditioned matrix, only a small number of prefixes are ``important''.
\begin{theorem}
	Given any matrix $A$ with an online condition number $\kappa^{\OL}$, there is a set $P = \set{i_1,\ldots,i_r} \subseteq [n]$, $i_1 < i_2 < \ldots < i_r$ of size $r = O((d\log n\kappa^{\OL})^{\max(p/2,1)}(d\log d + \log n))$ such that if $i \in [n]$ satisfies $i_j < i <  i_{j+1}$, then for all $x$,
\begin{align*}
	(1/4)\lp{A_{1:i}x} \le \lp{A_{1:{i_j}}x} \le \lp{A_{1:i}x}.
\end{align*}
	\label{thm:partition-theorem}
\end{theorem}

==> prelims.tex <==
Recall that given a matrix $A$ and a row $a_i$ of $A$, the offline $\ell_p$ sensitivity $\tau_i^{\ell_p}(A)$ is $\max_x |\la a_i, x\ra|^p/\lp{Ax}^p$ and online $\ell_p$ sensitivity $\tau_i^{\OL, \ell_p}(A)$ is $\max_x |\la a_i, x\ra|^p/\lp{A_{1:i}x}^p$. For any $n \times d$ matrix $A$ of rank $d$, $
    \sum_{i=1}^n \tau_i^{\ell_p}(A) \le d^{\max(p/2,1)}.
$
which can be proved using Lewis weights \cite{Lewis1978, cohen2015lp,woodruff2022online}. The sum of online $\ell_p$ sensitivities
\begin{align*}
    \sum_{i=1}^n \tau_i^{\OL, \ell_p}(A) \le O((d \log n\kappa^{\OL}(A))^{p/2}\log n).
\end{align*}
See Theorem~\ref{thm:bound-on-sum-of-online-sensitivities}.

Due to space constraints, all the proofs and additional explanations are moved to the Appendix.


==> removed.tex <==
\section{\texorpdfstring{$\ell_p \rightarrow \ell_\infty$}{lp to l\_infty} embedding using exponential random variables}
Let $A$ be an arbitrary $n \times d$ matrix and let $\bD$ be a random diagonal matrix with $\bD_{ii} = 1/\bE_i^{1/p}$, where $\bE_1,\ldots,\bE_n$ are standard exponential random variables. We now have the following standard lemma which states the max-stability property of exponential random variables.
\begin{lemma}
	If $\lambda_1,\ldots,\lambda_n > 0$ and $\bE_1,\ldots,\bE_n$ are independent standard exponential random variables, then
	\begin{align*}
		\max(\lambda_1/\bE_1,\ldots,\lambda_n/\bE_n) \equiv (\sum_i \lambda_i)/\bE
	\end{align*}
	where $\bE$ is also a standard exponential random variable.
\end{lemma}
Applying the above lemma, we have that for a fixed vector $x$, with $\bD$ as defined above, $\linf{\bD x}^p = \max_i |x_i|^p/\bE_i$ is distributed as $\lp{x}^p/\bE$. Using this property, we show that the matrix $\bD$ linearly embeds column space of $A$ into an $\ell_\infty$ space with low distortion. First, we have the following lemma that states that with high probability, for all $x$, $\linf{\bD Ax}$ is not too large compared to $\lp{Ax}$.
\begin{lemma}
	With probability $\ge 1-\delta$, for all $x$, \[\linf{\bD Ax} \le \frac{d^{\max(1/2+2/p, 1+1/p)}}{\delta^{1/p}}\lp{Ax}.\]
\end{lemma}
\begin{proof}
	We prove this by the standard way of using a well-conditioned basis to show that the matrix $\bD$ doesn't overestimate the $\ell_p$ norm of $Ax$ by a lot. Let $U$ be a $(d, d^{\max(1/2,1-1/p)},p)$ well-conditioned basis constructed using the L\"owner-John ellipsoid for column space of $A$. Consider an arbitrary $x \in \R^d$:
	\begin{align*}
		\linf{\bD Ux} &= \linf{\bD \sum_{i=1}^d U_{*i}x_i} \le \sum_{i=1}^d \linf{\bD U_{*i}}|x_i|\\
		&\le \left(\sum_{i=1}^d \linf{\bD U_{*i}}^p\right)^{1/p}\left(\sum_{i=1}^d |x_i|^q\right)^{1/q}\\
		&\le \left(\sum_{i=1}^d \linf{\bD U_{*i}}^p\right)^{1/p} d^{\max(1/2, 1-1/p)}\lp{Ux}.
	\end{align*}
	Here we used the Holder's inequality and that the fact that $U$ is a well-conditioned basis. Thus, it is now enough to bound $\sum_{i=1}^d \linf{\bD U_{*i}}^p$. From max-stability of exponential random variables, we have $\linf{\bD U_{*i}}^p$ is distributed as $\lp{U_{*i}}^p/\bE$. Using the fact that $\Pr[\bE \le \delta_1] \le \delta_1$, we obtain that
	\begin{align*}
	\Pr[\linf{\bD U_{*i}}^p \le \frac{\lp{U_{*i}}^p}{\delta_1}]	\ge 1 - \delta_1.
	\end{align*}
By a union bound over all $d$ columns of $U$, we obtain that with probability $\ge 1 - d\delta_1$,
\begin{align*}
	\sum_{i=1}^d \linf{\bD U_{*i}}^p \le \frac{\sum_{i=1}^d \lp{U_{*i}}^p}{\delta_1} \le d/\delta_1.
\end{align*}
Setting, $\delta_1 = \delta/d$, we obtain that with probability $\ge 1- \delta$, for all $x$,
\begin{align*}
	\linf{\bD Ux} \le (d^2/\delta)^{1/p}d^{\max(1/2,1-1/p)}\lp{Ux}.&\qedhere
\end{align*}
% Additional & required because of an amsthm bug with \qedhere
\end{proof}
\begin{lemma}
Given any $n \times d$ matrix $A$, let $\bD$ be the random diagonal matrix with each diagonal entry $\bD_{ii}$ set to be $1/\bE_i^{1/p}$ where $\bE_1,\ldots,\bE_n$ are independent standard exponential random variables. Then with probability $\ge 1 - \delta$, for all $x$,
\begin{align*}
	\frac{\lp{Ax}}{C(d\log(d/\delta))^{1/p}} \le \linf{\bD Ax} \le \frac{Cd^{\max(1/2+2/p,1+1/p)}}{\delta^{1/p}}\lp{Ax},
\end{align*}
where $C$ is a large enough absolute constant.
\label{lma:lp-to-linf-embedding}
\end{lemma}
\begin{proof}
	Let $U$ be the well-conditioned basis computed using the L\"owner-John ellipsoid. Let $x \in \R^d$ be arbitrary. We have $\linf{\bD Ux}^p$ is distributed as $\lp{Ux}^p/\bE$. From the cdf of exponential distribution, $\Pr[\bE \ge t] = e^{-t}$ for all $t$ which implies that
	\begin{align*}
		\Pr[\linf{\bD Ux}^p \le \delta_1\lp{Ux}^p] \le \exp(-1/\delta_1).
	\end{align*}
	Consider the set $S = \setbuilder{x \in \R^d}{\lp{Ux}=1}$. The set $S$ lies in the $\ell_2$ ball of radius $\sqrt{d}$ as $U$ is constructed using the L\"owner-John ellipsoid and hence satisfies for all $x$ that $(1/\sqrt{d})\opnorm{x} \le \lp{Ux}$. Now consider a set $N$ which forms a $\delta_2$ net for the set $S$ i.e., for every $x \in S$, there exists $y_x \in N$ such that $\opnorm{x - y_x} \le \delta_2$. By a greedy construction, we obtain a net $N$ of size
	\begin{align*}
		|N| \le (1 + \sqrt{d}/\delta_2)^d = \exp(2d\log(\sqrt{d}/\delta_2)).
	\end{align*}
	Setting $\delta_1 = \frac{1}{2d\log(\sqrt{d}/\delta_2)+\log(1/\delta_3)}$, by a union bound over the net $N$, we obtain that with probability $\ge 1 - \delta_3$, for all $y \in N$,
	\begin{align*}
		\linf{\bD Uy}^p \ge \frac{\lp{Uy}^p}{2d\log(\sqrt{d}/\delta_2) + \log(1/\delta_3)} = \frac{1}{2d\log(\sqrt{d}/\delta_2) + \log(1/\delta_3)}
	\end{align*}
	which implies that with probability $\ge 1 - \delta_3$, for all $y \in N$,
	\begin{align*}
		\linf{\bD Uy} \ge \frac{1}{(2d\log(\sqrt{d}/\delta_2) + \log(1/\delta_3))^{1/p}}.
	\end{align*}
	By union bound, with probability $\ge 1 - \delta_3 - \delta_4$, we have that both the above property and the property that for all $x$,
	\begin{align*}
		\linf{\bD Ux} \le \frac{d^{\max(1/2+2/p, 1+1/p)}\lp{Ux}}{\delta_4^{1/p}},
	\end{align*}
	hold. Now, for an arbitrary $x \in S$, by triangle inequality,
	\begin{align*}
		\linf{\bD Ux} &\ge \linf{\bD Uy_x} - \linf{\bD U(x-y_x)}\\
		&\ge \frac{1}{(2d\log(\sqrt{d}/\delta_2) + \log(1/\delta_3))^{1/p}} - \frac{d^{\max(1/2+2/p,1+1/p)}}{\delta_4^{1/p}}\lp{U(x-y_x)}\\
		&\ge \frac{1}{(2d\log(\sqrt{d}/\delta_2) + \log(1/\delta_3))^{1/p}} - \frac{d^{\max(1/2+2/p,1+1/p)}}{\delta_4^{1/p}}\opnorm{x-y_x}\\
		&\ge \frac{1}{(2d\log(\sqrt{d}/\delta_2) + \log(1/\delta_3))^{1/p}} - \frac{d^{5/2}}{\delta_4^{1/p}}\delta_2.
	\end{align*}
	In the above sequence of inequalities, we used the fact that for all $x$, we have $\lp{Ux} \le \opnorm{x}$. Setting $\delta_3 = \delta_4 = \delta/2$ and $\delta_2 = O(\delta^{1/p}/\poly(d,\log(1/\delta)))$, we obtain that with probability $\ge 1 - \delta$, for all vectors $x$,
	\begin{align*}
		\frac{\lp{Ux}}{C(d\log(d/\delta))^{1/p}} \le \linf{\bD Ux} \le \frac{Cd^{\max(1/2+2/p, 1+1/p)}}{\delta^{1/p}}\lp{Ux}.
	\end{align*}
	for a large enough constant $C$.
\end{proof}

==> turnstile.tex <==
Recall the streaming model with deletions as described in the introduction. We receive $n$ requests of the form ``insert/delete $a_i$'' where $a_i \in \set{-M, \ldots, M}^d$ for $M = \poly(d)$. We also assume that for each row, the number of deletions does not exceed the number of insertions. For each row candidate $a \in \set{-M, \ldots, M}^d$, let $\freq(a)$ denote the difference between the number of ``insert $a$'' and the number of ``delete $a$'' requests. We assume that for all $a$, $\freq(a) \ge 0$. Let $r$ denote the number of rows $a$ with $\freq(a) > 0$. Thus, $\dedup(A) \in \R^{r \times d}$ is the matrix formed by all the rows $a$ with $\freq(a) > 0$. We also have that $r \le n$. Let $b_1,\ldots,b_r$ be the rows of the matrix $\dedup(A)$. We construct an $\ell_p$ subspace embedding for the matrix $\dedup(A)$ using sub-linear space by making $O(\log (n))$ passes over the stream.

As the rows $a_i$ have integer coordinates of absolute value at most $M$, we have that there are only at most $(2M+1)^d$ distinct possible rows that appear in the stream. Thus, the turnstile stream of rows can be considered as updating an $N = \poly(n)^d$ dimensional vector in a stream with $\pm 1$ updates to an appropriate coordinate depending on whether a row $a_i$ is being inserted or deleted.

We use $\ell_0$ sampling algorithms in a stream and $\ell_p$ sensitivity sampling to show that an $\ell_p$ subspace embedding for matrix $\dedup(A)$ can be constructed by making $O(\log n)$ passes over the stream. We first state the following results which we use throughout.

\begin{theorem}[{\cite[Theorem~10]{kane2010optimal}}]
Given a stream of updates $(i_1, v_1), (i_2, v_2), \ldots,(i_m, v_m) \in [N] \times \set{-M, \ldots, M}$ to an $n$ dimensional vector $x$ initialized to $0$, there is a ``linear'' streaming algorithm that $1 \pm \varepsilon$ approximates $L_0(x) = |\supp(x)|$ using a space of $O(\varepsilon^{-2}\log N(\log 1/\varepsilon + \log\log mM))$ bits.
\label{thm:count-approximation}
\end{theorem}

Using the natural encoding of a row $a_i$ as an integer in $[N]$, using the above algorithm, we can obtain a $1+\varepsilon$ approximation to the number of rows in $\dedup(A)$ using $O(\varepsilon^{-2} d \log(n)(\log (1/\varepsilon)+ \log d +\log\log n))$ bits of space.

\begin{theorem}[{\cite[Theorem~2]{JST11}}]
Given a turnstile stream of updates to an $N$-dimensional vector $x$ initialized to all $0$s, there is a zero relative error ``linear'' $\ell_0$ sampler with additive error $\Delta = O(N^{-c})$ and $\delta$ failure probability that takes $O(\log^2 N \log 1/\delta)$ bits of space. The update time and recovery time of the algorithm is $O(\log N)$.
\label{thm:l0-sample}
\end{theorem}
Given a turnstile stream of updates $(i_1,v_1), \ldots, (i_m,v_m) \in [N] \times \set{-M, \ldots, M}$, let $x \in \R^N$ be the underlying vector at the end of the stream. The above algorithm with probability $\ge 1 - \delta$, outputs an index $\bi \in \supp(x)$ such that with probability $\ge 1 - \delta$, 
    $\Pr[\bi = i] = {1}/{|\supp(x)|} \pm N^{-c}$ for all $i \in \supp(x)$. Using $O(\poly(d, \log n)\log(1/\delta))$ bits of space, we can thus sample from a distribution close to the uniform distribution over the rows in $\dedup(A)$.

The term ``linear'' here means that the algorithms maintain a linear sketch of the stream and, at the end of the stream, based on the linear sketch outputs an estimation or a sample.
\subsection{Recursive \texorpdfstring{$\ell_p$}{lp} sensitivity sampling}
\begin{algorithm}
    \KwIn{A matrix $A \in \R^{n \times d}$, a parameter $p \in [1, \infty)$ and $\varepsilon$}
    \KwOut{A matrix $M$ that satisfies with probability $\ge 99/100$ that for all $x \in \R^{d}$, $\lp{Mx}^p = (1 \pm \varepsilon)\lp{Ax}^p$.}
If $n \le \poly(d)$, return $A$\;
$\bS \gets $ A random subset of $[n]$ obtained by sampling each $i \in [n]$ to be in set $\bS$ with probability $1/2$\;
$M_{\bS} \gets $ Recursively obtain a subspace embedding for $A_{\bS}$ with accuracy parameter $\varepsilon = 1/2$ and sample parameter $s$\;
For $i \in [n]$, define $\tau_i^{M_\bS} := \min(1, \max_x |\la a_i, x\ra|^p/\lp{M_{\bS}x}^p)$\;
Sample $d^{O(p)}\poly(\log n)/\varepsilon^2$ rows from $A$ independently with probabilities proportional to $\tau_i^{\bS}$ and form $M$ by appropriately scaling the sampled rows\;
\Return{M}
\caption{Recursive $\ell_p$ Sensitivity Sampling}\label{alg:recursive-sampling-algorithm}
\end{algorithm}
Algorithm~\ref{alg:recursive-sampling-algorithm} is a recursive algorithm to compute approximate $\ell_p$ sensitivities and sample from a distribution based on the approximate sensitivities. The recursive sampling procedure was earlier used in \cite{cohen2015uniform} and \cite{cohen2015lp} to construct $\ell_2$ and $\ell_p$ subspace embeddings respectively. While the earlier works were more concerned about constructing subspace embeddings in near input-sparsity time, we use the above algorithm as it is amenable to implementation in a stream with duplicates. We make a slight modification to the proof of \cite{cohen2015uniform} to allow for independently sampling each coordinate to be in a random subset instead of drawing a uniform random subset with half the entries of the original set. We can now show that this simple recursive algorithm can be implemented by making $O(\log n)$ passes over the stream. 
% \subsection{Formalizing the stream}
% In the stream, we receive updates of the form (i) add $a$, and (ii) delete $a$ for vectors $a \in \set{-M, \ldots, M}^d$. We assume that $M \le \poly(n)$. We assume that for any $a$, the number of delete requests is at most the number of add requests $a$. Let $a_1,\ldots,a_m$ be the distinct rows that appear in the stream with counts $c_1,\ldots,c_m$ where $c_i$ denotes the difference between the number of add and delete requests for the row $a_i$. Hence $c_i \ge 0$ from our assumption. Without loss of generality let $n \le m$ be the integer such that $c_1,\ldots,c_n > 0$ and $c_{n+1},\ldots,c_m = 0$. Our aim is to construct an $\ell_p$ subspace embedding for the matrix $A$ with rows given by $a_1,\ldots,a_n$. 
\subsection{Implementing the Algorithm in a stream}
Unwinding the recursion in Algorithm~\ref{alg:recursive-sampling-algorithm}, we obtain that the algorithm recursively sub-samples the rows of the matrix and uses the subspace embedding computed in an iteration to obtain sensitivity estimates of rows in the next iteration and then sample from that distribution.

To implement it in the context of streams with deletions, we therefore need to be able to recursively sub-sample the rows of the deduplicated matrix and given a subspace embedding for the sub-sampled deduplicated matrix in iteration $j$, we need to be able to compute a subspace embedding for the sub-sampled deduplicated matrix in iteration $j+1$. We use fully random hash functions to obtain recursively sub-sampled rows of the deduplicated matrix. We show that the ``fully random'' assumption can be removed and hash functions generated by Nisan's pseudorandom generator \cite{nisan1990pseudorandom} suffice using a standard derandomization argument.

Now suppose we have a subspace embedding for the sub-sampled deduplicated matrix in the $j$-th iteration. We now want to sample rows of the deduplicated matrix in the $(j+1)$-th iteration from an appropriate distribution. For each row in the stream, we compute the probability with which we want to sample the row and partition the rows into buckets based on the probabilities. Within each bucket, we use the $\ell_0$ sampling algorithm to sample a random row from the deduplicated matrix in the $(j+1)$-th iteration that falls in the bucket. By maintaining multiple independent $\ell_0$ samplers, we show that rows from the deduplicated matrix in the $(j+1)$-th iteration can be sampled using an appropriate distribution. See the appendix for more details.
\begin{theorem}
For a constant $p>1$, given a stream ``insert/delete $a_1$'', \ldots, ``insert/delete $a_n$'' with $a_i \in \set{-M, \ldots, M}^d$ for $M = \poly(n)$, there is a streaming algorithm that makes $O(\log n)$ passes over the requests that uses $d^{O(p)}\poly(\log n)/\varepsilon^2$ bits of space and outputs an $\varepsilon$ $\ell_p$ subspace embedding for $\dedup(A)$.
\label{thm:logn-round-subspace-embedding}
\end{theorem}

Note that Algorithm~\ref{alg:recursive-sampling-algorithm} samples around half of the rows in the input matrix in each recursive call. If we instead sample just a $1/n^{1/t}$ fraction of rows, the same algorithm can be implemented in $O(t)$ rounds using $n^{1/t}\poly(d, \log n)/\varepsilon^2$ bits of space.

